Efficacy of Satisfiability Based Attacks in the Presence of Circuit Reverse Engineering Errors

Intellectual Property (IP) theft is a serious concern for the integrated circuit (IC) industry. To address this concern, logic locking countermeasure transforms a logic circuit to a different one to obfuscate its inner details. The transformation caused by obfuscation is reversed only upon application of the programmed secret key, thus preserving the circuit's original function. This technique is known to be vulnerable to Satisfiability (SAT)-based attacks. But in order to succeed, SAT-based attacks implicitly assume a perfectly reverse-engineered circuit, which is difficult to achieve in practice due to reverse engineering (RE) errors caused by automated circuit extraction. In this paper, we analyze the effects of random circuit RE-errors on the success of SAT-based attacks. Empirical evaluation on ISCAS, MCNC benchmarks as well as a fully-fledged RISC-V CPU reveals that the attack success degrades exponentially with increase in the number of random RE-errors. Therefore, the adversaries either have to equip RE-tools with near perfection or propose better SAT-based attacks that can work with RE-imperfections.

==> casestudy.tex <==
\subsection{Case study with \texttt{c880}}
\label{sec:case-study}

%\subsection{Other types of reverse-engineering error that do not contribute to security}

\Aysuworries{Let's combine all single reverse engineering errors into a single figure.}
Figures~\ref{fig:nandtoxnor},~\ref{fig:nandtoxor} and~\ref{fig:nortoxor} show cases in \texttt{c880} circuit, with other types of single reverse-engineering errors and how the SAT-solver nullifies their effects through suitable key search. 
\begin{figure}[!h]
    \centering
    %\vspace{-3in}
    \includegraphics[scale=0.45]{fig/nandtoxnor.eps}
    \caption{NAND$\rightarrow$XNOR}
    \label{fig:nandtoxnor}
\end{figure}
\begin{figure}[!h]
    \centering
    %\vspace{-3in}
    \includegraphics[scale=0.45]{fig/nandtoxor.eps}
    \caption{NAND$\rightarrow$XOR}
    \label{fig:nandtoxor}
\end{figure}
%\begin{figure}[!h]
%    \centering
%    %\vspace{-3in}
%    \includegraphics[scale=0.45]{fig/nortoxnor.eps}
%    \caption{NOR$\rightarrow$XNOR}
%    \label{fig:nortoxnor}
%\end{figure}
\begin{figure}[!h]
    \centering
    %\vspace{-3in}
    \includegraphics[scale=0.45]{fig/nortoxor.eps}
    \caption{NOR$\rightarrow$XOR}
    \label{fig:nortoxor}
\end{figure}


%\begin{figure}[!h]
%    \centering
%    %\vspace{-3in}
%    \includegraphics[scale=0.45]{fig/xnor_key0_1.eps}
%    \caption{XNOR with $key=0$}
%    \label{fig:xnor_key0}
%\end{figure}

%\begin{figure}[!h]
%    \centering
%    %\vspace{-3in}
%    \includegraphics[scale=0.45]{fig/xnor_key1_1.eps}
%    \caption{XNOR$\rightarrow$XOR}
%    \label{fig:xnortoxor}
%\end{figure}

%\begin{figure}[!h]
%    \centering
%    %\vspace{-3in}
%    \includegraphics[scale=0.45]{fig/xor_key0.eps}
%    \caption{XOR$\rightarrow$XNOR}
%    \label{fig:xortoxnor}
%\end{figure}

%\begin{figure}[!h]
%    \centering
%    %\vspace{-3in}
%    \includegraphics[scale=0.45]{fig/xor_key1.eps}
%    \caption{XOR with $key=1$}
%    \label{fig:xor_key1}
%\end{figure}


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}




==> threat-model.tex <==
%\begin{figure}[!t]
%    \centering
%    \vspace{-0.6in}
%    \includegraphics[scale=0.3, left]{fig/RE-attack-model.pdf}
%    \vspace{-0.9in}
%    \caption{Threat Model}
%    \vspace{-0.2in}
%    \label{fig:threat-model}
%\end{figure}








%\subsection{Threat Model}
%\label{sec:threat-model}
%The adversary is the end-user who purchases the product/IC from the open market. The end user corresponds to an attacker who has access the product, and who depackages, delayers and uses imaging techniques to perform automated circuit extraction.
%\Aysuworries{Could we add a sentence to rebuke the "end of logic locking" paper or can anyone would just simply say logic locking threat model is useless?}






